Histopathological Cancer Detection Using Hybrid Quantum Computing

We present an effective application of quantum machine learning in the field of healthcare. The study here emphasizes on a classification problem of a histopathological cancer detection using quantum transfer learning. Rather than using single transfer learning model, the work model presented here consists of multiple transfer learning models especially ResNet18, VGG-16, Inception-v3, AlexNet and several variational quantum circuits (VQC) with high expressibility. As a result, we provide a comparative analysis of the models and the best performing transfer learning model with the prediction AUC of approximately 93 percent for histopathological cancer detection. We also observed that for 1000 images with Resnet18, Hybrid Quantum and Classical (HQC) provided a slightly better accuracy of 88.5 percent than classical of 88.0 percent.

==> data.tex <==
\section{data}
 The dataset used for this work is a set of digital pathology images from the benchmark dataset know as
 PatchCamelyon(PCam) \cite{Veeling2018-qh}. This is a large-scale patch-level dataset derived from Camelyon16 \cite{babak2017diagnostic} data. The aggregate of the patches make up the slide-level image, which can be used to predict likelihood of metastases, stage cancer. 


\begin{figure*}[htbp]
\centerline{\includegraphics{images/0_value.jpg}}
%\centerline{\includegraphics[width=17cm]{images/1_value.jpg}}
\caption{Data Samples}
\label{fig:sim}
\end{figure*}  



 
 
